PHASOR: Phase-Anchored Universal Action Representations for Humanoid Embodiments

Learning a good action embedding space is fundamental to scalable robot policy learning, yet existing methods treat action latents as task-specific intermediates rather than first-class representations. The resulting latents are unstructured, embodiment-specific, and weakly tied to motion semantics, limiting interpretability, controllability, and transferability across robots. We position the action embedding space itself as a first-class design target, with downstream policy quality emerging from representation quality. Exploiting motion's intrinsic periodicity, we factorize it into a phase manifold that captures cyclic structure via FFT-parametric coefficients, together with a pose branch that conditions the manifold on non-periodic configuration detail. Combined with motion-semantic distillation, this factorized structure yields a cross-embodiment motion manifold that is interpretable and embodiment-agnostic by design. Anchoring multiple humanoid robots to a shared human-pretrained manifold then produces a unified action embedding space across diverse platforms, achieving strong cross-embodiment retrieval and consistent gains on downstream robot tasks.

==> tables/exp_downstream.tex <==
% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{l cc cc}
% \toprule
%  & \multicolumn{2}{c}{\textbf{Task 1: Imitation}} & \multicolumn{2}{c}{\textbf{Task 2: Teleoperation}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% \textbf{Variant} & $d_z$ & MPJPE$\downarrow$ & $d_z$ & MPJPE$\downarrow$ \\
% \midrule
% Proprioceptive raw & (Robot, 295D) & 1.83 & (Human, 132D) & 64.85 \\
% MLP                & 80  & 1.83             & 80  & 66.79 \\
% VQ                 & 10  & \underline{1.69} & 10  & 65.17 \\
% \rowcolor{blue!10}
% \textbf{PHASOR}    & 64  & \textbf{1.62}    & 64  & \textbf{64.75} \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Downstream results.} All encoders frozen, only the policy head trained. The first row drives the head from raw proprioceptive input with no learned embedding. MPJPE in mm ($\downarrow$).}
% \label{tab:downstream}
% \end{table*}% % % % % % % % % % % % % % % % % % % % 

% tables/exp_downstream.tex
% \begin{table}[t]  ← 이 줄 제거
% \centering        ← 이 줄 제거
\resizebox{0.75\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Task 1: Imitation}} 
 & \multicolumn{2}{c}{\textbf{Task 2: Teleoperation}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\textbf{Variant} & $d_z$ & MPJPE$\downarrow$ & $d_z$ & MPJPE$\downarrow$ \\
\midrule
Proprioceptive raw & (Robot, 295D) & 1.83 & (Human, 132D) & 64.85 \\
MLP                & 80           & 1.83 & 80            & 66.79 \\
VQ                 & 10           & 1.69 & 10            & 65.17 \\
\textbf{PHASOR}    & 64           & \textbf{1.62} & 64 & \textbf{64.75} \\
\bottomrule
\end{tabular}}
% \end{table}  ← 이 줄 제거

==> tables/exp_summary.tex <==
\begin{table}[t]
\centering

\label{tab:summary}
\small
\begin{tabular}{llccc}
\toprule
\textbf{Experiment} & \textbf{Metric} & \textbf{PHASOR} & \textbf{Best Baseline} & $\Delta$ \\
\midrule
Retrieval H$\to$R & win mAP$\uparrow$   & \textbf{0.233} & MLP\;\;0.208   & +12.0\% \\
Retrieval R$\to$R & win mAP$\uparrow$   & \textbf{0.223} & SONIC\;0.206   & +8.3\%  \\
Imitation         & MPJPE mm$\downarrow$ & \textbf{1.56}  & SONIC\;1.69    & $-$7.7\%  \\
Teleoperation     & MPJPE mm$\downarrow$ & \textbf{64.55} & raw\;\;64.85   & $-$0.5\%  \\
RL Locomotion     & Phase cos$\uparrow$  & --             & --             & TBD     \\
\bottomrule
\end{tabular}
\caption{Consolidated results. $\uparrow$\,=\,higher is better; $\downarrow$\,=\,lower is better. Best in \textbf{bold}.}
\end{table}

==> tables/tmp.tex <==
% tables/exp_retrieval_main.tex
\begin{table*}[t]
\centering
\label{tab:retrieval_main}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.07}
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{l | cccc | cccc | cccc}
\toprule
 & \multicolumn{4}{c|}{\textbf{H$\to$R Exact}} & \multicolumn{4}{c|}{\textbf{R$\to$H Exact}} & \multicolumn{4}{c}{\textbf{R$\to$R Exact}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Method & R@1 & R@5 & R@10 & MRR & R@1 & R@5 & R@10 & MRR & R@1 & R@5 & R@10 & MRR \\
\midrule
\multicolumn{13}{l}{\emph{Baselines}} \\
\midrule
MLP \citep{...}                  & 79.9 & 96.5 & 98.8 & 87.1 & 79.8 & \underline{97.5} & \underline{99.3} & 87.4 & 74.7 & \underline{95.0} & \underline{98.2} & \underline{83.5} \\
VQ \citep{...}
                                  & 37.6 & 78.6 & 91.0 & 55.1 & 36.3 & 77.0 & 89.5 & 53.6 & 37.5 & 77.7 & 89.8 & 54.8 \\
\midrule
\multicolumn{13}{l}{\emph{PHASOR (A) Alignment loss design}} \\
\midrule
Only Phase \,(no cross-emb training)         & 83.0 & 91.9 & 93.6 & 87.0 & 83.9 & 92.2 & 94.1 & 87.8 & 73.0 & 84.3 & 87.3 & 78.2 \\
Hard only (no LAMP)                          & 84.1 & 92.2 & 93.8 & 87.8 & 84.1 & 92.5 & 94.2 & 87.8 & 74.5 & 85.3 & 88.1 & 79.5 \\
\;\;$+$ Soft Clip (C\textsubscript{2})        & 84.9 & 92.7 & 94.3 & 88.5 & 85.1 & 93.0 & 94.6 & 88.6 & 76.1 & 86.4 & 88.9 & 80.7 \\
\;\;$+$ Soft Window (W)                       & 85.6 & 93.4 & 94.9 & 89.1 & 85.7 & 93.7 & 95.2 & 89.1 & 77.2 & 87.1 & 88.6 & 81.6 \\
\;\;$+$ Soft Hierarchical (W $+$ C)           & 86.9 & 94.3 & 95.8 & 89.9 & 87.2 & 94.8 & 96.3 & 90.2 & 79.3 & 89.6 & 91.8 & 83.7 \\
\midrule
\multicolumn{13}{l}{\emph{PHASOR (B) Alignment target}} \\
\midrule
$\pi(\mathbf{P}_\tau \,\|\, X_\text{root})$ \;($+$ raw root pose)
                                              & \underline{88.5} & \underline{96.0} & \underline{97.2} & \underline{91.9} & \underline{89.5} & 96.5 & 97.5 & \underline{92.6} & \underline{81.0} & 91.7 & 93.9 & 85.8 \\
\textbf{$\pi(\mathbf{P}_\tau \,\|\, z_\text{pose}^\text{mod,pool})$\; (Ours)}
                                              & \textbf{90.3} & \textbf{98.3} & \textbf{99.2} & \textbf{93.9} & \textbf{90.5} & \textbf{98.6} & \textbf{99.4} & \textbf{94.1} & \textbf{84.8} & \textbf{96.4} & \textbf{98.3} & \textbf{90.0} \\
\bottomrule
\end{tabular}}
\caption{Cross-embodiment exact-match retrieval and PHASOR design ablation on our val set. Each query has exactly one positive: the temporally identical chunk from a different embodiment.
  \textbf{Directions}: H$\to$R (human query $\to$ robot, avg.\ G1/H1.2/T1/BHL), R$\to$H (robot $\to$ human, avg.\ four robots), R$\to$R (robot $\leftrightarrow$ robot, avg.\ $\binom{4}{2}{=}6$ pairs, both directions).
  \textbf{Baselines}: \emph{MLP}: per-embodiment feature projection with InfoNCE. \emph{VQ Codebook (LAPA-family)}: finite-scalar-quantized codebook encoder-decoder with cross-reconstruction.
  \textbf{(A) Alignment loss.} \emph{Only Phase}: phase manifold trained only on human (frozen, applied zero-shot to robots, no cross-emb training). \emph{Hard only} adds cross-embodiment InfoNCE on top. Adding LAMP-derived soft targets (Soft Clip, Soft Window) each improves; their hierarchical combination is best.
  \textbf{(B) Alignment target.} Holding loss $=$ Soft Hierarchical, concatenating raw root pose at the alignment head input ($+$1.6\,pt R@1) and replacing it with the pooled, FiLM-modulated $z_\text{pose}^\text{mod}$ (Ours, $+$1.8\,pt) progressively improves alignment, with the latter dominating all metrics across all three directions. Pose decoupling (auxiliary $R_\text{joint}/X_\text{root}$ branch with bidirectional FiLM) is held \cmark throughout (A) and (B) as a structural assumption of PHASOR.
  All values in \%. \textbf{Bold}: best per column. \underline{Underline}: second best.}
\end{table*}

